SE(3)-DiffusionFields: Learning smooth cost functions for joint grasp and motion optimization through diffusion

Multi-objective optimization problems are ubiquitous in robotics, e.g., the optimization of a robot manipulation task requires a joint consideration of grasp pose configurations, collisions and joint limits. While some demands can be easily hand-designed, e.g., the smoothness of a trajectory, several task-specific objectives need to be learned from data. This work introduces a method for learning data-driven SE(3) cost functions as diffusion models. Diffusion models can represent highly-expressive multimodal distributions and exhibit proper gradients over the entire space due to their score-matching training objective. Learning costs as diffusion models allows their seamless integration with other costs into a single differentiable objective function, enabling joint gradient-based motion optimization. In this work, we focus on learning SE(3) diffusion models for 6DoF grasping, giving rise to a novel framework for joint grasp and motion optimization without needing to decouple grasp selection from trajectory generation. We evaluate the representation power of our SE(3) diffusion models w.r.t. classical generative models, and we showcase the superior performance of our proposed optimization framework in a series of simulated and real-world robotic manipulation tasks against representative baselines.

==> sections/limitations.tex <==


\begin{enumerate}
    \item pointcloud as perception input
    \item computation time
    \item for now, we only learn fixed energies and do not improve / optimize them, given the collected data
\end{enumerate}

==> sections/rest.tex <==
% maybe some more general introduction: (PROBLEM FORMULATION)
Physical object interaction, and in particular grasping, is a crucial skill for intelligent, autonomous robotic systems. Yet, despite the practical and scientific relevance, 6D object grasping remains challenging (say something like: 1) difficult to deal with objects of different shapes / to generalize, 2) having to deal with potentially cluttered scenes,i.e., have to take the motion into account, 3) perhaps only partially observable, 4) for many taks, grasp has to be conditioned on the downstream task of interest, which is often not reflected in related work).
Therefore the focus of paper is mainly two-fold - 1) learning powerful, implicit energy functions for versatile grasp pose generation; 2) combining multiple energy-based functions in an optimization framework to achieve task-conditioned grasping, a skill that is not often studied in related work,...

% Niklas: sorry for non smooth transition, but I think I would approach it from here and then continue with what you put already, Julen

In this paper, we study the problem of learning grasp pose generative models. In contrast with previous methods that consider explicit or semi-explicit generative models, we propose to model the generative model by an energy/cost function that will represent the quality of a particular SE(3) pose. This modular formulation allows for multi-objective optimization, exemplary, optimizing the grasp pose while already considering a desired placing pose. We introduce a model to represent the implicit function, show a proper way to train it and present and evaluate a set of interesting properties of implicit grasps generative models that are unique from considering a fully implicit function to represent the grasp generator.

Most common grasp generative models assume a direct approach to generate grasps. Grasp-Net trains a Variational Auto-encoder to represent the grasp pose distribution. To generate grasp samples, a noise signal is input into the decoder and a grasp pose is obtained as output
\begin{align}
    \mH_{g} = \mG_{\vtheta}(\vz) \, , \, \vz \sim \gN(\vzero,\mI).
\end{align}
We call explicit functions to these functions. Another common approach are the semi-explicit models. These models assume an implicit function that outputs the quality of a query 3D position for the gripper. The function provides low cost to those 3D positions that are good for grasping and generate the optimal grasp orientation explicitly for a given 3D point.

In complex manipulation tasks, the grasp generative models are combined with additional objectives by first, sampling a set of grasp candidates and then, evaluating the quality of the candidates on the additional costs or computing inverse kinematics on the grasp candidates to find feasible robot joint configurations.

In contrast with previous approaches, we propose representing the grasp generative model by an implicit function
\begin{align}
    c = \mE_{\vtheta}(\mH_g).
\end{align}
Differing from explicit functions, we can not sample directly from an implicit function. An implicit function outputs a cost value that represents the quality of query grasp pose. To generate a sample, we are required to use some type of \gls{mcmc} methods over the implicit function.

Considering a fully implicit function has multiple interesting properties wrt. explicit functions. The implicit function can be easily composed with additional costs(both heuristic or learned) and optimize jointly over the sum of the costs. In contrast, explicit methods usually divide the problem between generating a set of grasp candidates and evaluating the quality of these grasps over a set of costs. Another interesting property is in the optimization spaces. Implicit functions allows to optimize directly in the configuration space of the robot by propagating the configuration to the task space, evaluate the grasp and propagate back the gradient over the costs by the Jacobian. In contrast, explicit methods require first to find the grasps in the task space and then apply inverse kinematics to find the optimal robot configuration. 

Additionally, in the last years, implicit function based generative models have outperformed explicit generative models in terms of both the quality of the generated samples and variability. While the implicit functions have been mainly applied for image generation, we hypothesize that implicit generative models can provide a higher variability and more accurate grasp poses with respect to the explicit functions.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ROBOT GRASP CONF %%%%%%%%%%%%%%%
\\
\textbf{Robot grasp configuration generation.}
We consider the problem of finding robot joint configurations resulting in successful and feasible grasps. This is a multi-objective optimization as successful solutions require compatibility of the desired grasp pose and the robot's workspace while avoiding table collisions. We propose solving the problem as a single optimization problem as presented in \cref{sec:optimization}. We exploit differentiable forward kinematics to map a robot configuration to the end effector's space (SE(3)) and evaluate grasp quality using \gls{se3dif}. We add additional cost terms and optimize the robot's joint configuration $\vq$ over the total set of costs (more details in \cref{app:rechability_eval}). The initial samples are sampled from a uniform distribution bounded by the joint limits'.
\\
As baselines we consider two methods. The first (joint opt - classifier) applies our proposed joint optimization scheme, yet replacing \gls{se3dif} with the trained classifier from \cref{sec:exp_grasp_gen}. The second (sample + opt), considers a separate two-stage optimization, in which we first sample SE(3) grasp poses using \gls{se3dif} as in the previous experiment.
%at \cref{app:grasp_generation_pseudocode}) 
This sampling neglects the robot's kinematic constraints and potential table collisions. In the second step, we optimize the robot's joint configuration to match the desired grasp poses from the first step and avoiding table collisions.
Such separate, multi-stage optimization procedures have previously been proposed for handling robot grasp pose generation in very similar settings and achieve state-of-the-art performance \cite{murali20206, lou2021collision, zhou20176dof, ten2017grasp, lu2020multifingered}.
\\
We report averaged results across all mugs considering $n_s{=}100$ initial samples and evaluate grasp quality by attempting to lift the mugs starting from the proposed robot configuration.
The results in Table \ref{table:robo_grasp_pose_generation1} reveal that across all experiments, our proposed joint optimization procedure results in the highest success rates $s_\Omega$ and $s_1$, i.e., considering evaluating all particles, and only the best one, respectively. 
In line with the previous results, the learned classifier's energy landscape is not suitable for gradient-based optimization and hence results in lowest successes.
The separate optimization (sample + opt) performs substantially better, but still worse compared to our proposed
\begin{table}[t]
\vspace{-10pt}
\begin{center}
\caption{Comparing different approaches for robot grasp pose generation with $n_s{=}100$ initial samples.}
\vspace{-0.2cm}
\scalebox{0.75}{
\label{table:robo_grasp_pose_generation1}
\begin{tabular}{l|cc|cc}
       & \multicolumn{2}{c|}{Objects upright} & \multicolumn{2}{c}{Objects flipped} \\
 Method          & $s_\Omega$ & $s_1$ & $s_\Omega$ & $s_1$ \\
\hline
\hline

joint opt (classifier) & 0.03 & 0.77 & 0.03 & 0.68 \\
sample (\gls{se3dif}) + opt    &0.46 & 0.80 &  0.12 &  0.76 \\
\textbf{\textbf{Ours}} & \textbf{0.62} & \textbf{0.88} & \textbf{0.49} & \textbf{0.88} \\
\hline

\end{tabular}
}
\end{center}
\vspace{-10pt}
\end{table}
joint optimization with \gls{se3dif}. Particularly, the experiments showcase a performance drop w.r.t. the flipped mug scenario. This underlines the major shortcoming of not being adaptive w.r.t. the current environment, i.e., sampling grasps which are simply infeasible. Contrarily, for our proposed method $s_\Omega$ drops only slightly, and $s_1$ even remains high at $0.88$.
We, thus, conclude that end-end gradient-based optimization with our \gls{se3dif} model results in highly performant, reliable, and adaptive robot grasp pose generation, despite the multi-objective scenario (more details in \cref{app:rechability_eval}).

\\
